Zeroth-Order Stochastic Variance Reduction for Nonconvex Optimization

As application demands for zeroth-order (gradient-free) optimization accelerate, the need for variance reduced and faster converging approaches is also intensifying. This paper addresses these challenges by presenting: a) a comprehensive theoretical analysis of variance reduced zeroth-order (ZO) optimization, b) a novel variance reduced ZO algorithm, called ZO-SVRG, and c) an experimental evaluation of our approach in the context of two compelling applications, black-box chemical material classification and generation of adversarial examples from black-box deep neural network models. Our theoretical analysis uncovers an essential difficulty in the analysis of ZO-SVRG: the unbiased assumption on gradient estimates no longer holds. We prove that compared to its first-order counterpart, ZO-SVRG with a two-point random gradient estimator could suffer an additional error of order $O(1/b)$, where $b$ is the mini-batch size. To mitigate this error, we propose two accelerated versions of ZO-SVRG utilizing variance reduced gradient estimators, which achieve the best rate known for ZO stochastic optimization (in terms of iterations). Our extensive experimental results show that our approaches outperform other state-of-the-art ZO algorithms, and strike a balance between the convergence rate and the function query complexity.

==> Supp_Main.tex <==

\section{Supplementary material}\label{sec: supp}

\subsection{Zeroth-order (ZO) gradient estimators}\label{supp: ZOgrad}
With an abuse of notation, in this section let $f$ be an arbitrary function under assumptions A1 and A2.
Lemma\,\ref{lemma: smooth_f_random} shows the second-order statistics of  \ref{eq: grad_rand}.

 

\begin{mylemma}
\label{lemma: smooth_f_random}
%\citep[Lemma\,4.1]{gao2014information}
Suppose that Assumption A1 holds, and define $f_\mu = \mathbb E_{\mathbf u \in U_{\mathrm{b}}}[f(\mathbf x + \mu \mathbf u)]$, where $U_{\mathrm{b}}$ is a uniform distribution over the unit Euclidean ball. Then  \ref{eq: grad_rand} yields:

1) $f_\mu$ is $L$-smooth, and
\begin{equation}\label{eq: smooth_est_grad}
    \nabla f_\mu (\mathbf x) 
    %  = \mathbb E_{\mathbf u }
    % \left [
    % \frac{d}{\mu} f(\mathbf x + \mu \mathbf u) \mathbf u
    % \right ] 
    =  \mathbb E_{\mathbf u }
    \left [
    \hat \nabla f(\mathbf x)
    \right ],
\end{equation}
where $\mathbf u$ is drawn from 
the uniform distribution over the unit Euclidean
sphere, and 
$\hat \nabla f(\mathbf x)$ is given by \ref{eq: grad_rand}.

2) For any $\mathbf x \in \mathbb R^d$,
\begin{align}
& | f_\mu(\mathbf x) - f(\mathbf x) | \leq \frac{L \mu^2}{2} \label{eq: dist_f_smooth_true_random}  \\
& \| \nabla f_\mu (\mathbf x) - \nabla f(\mathbf x) \|_2^2 \leq \frac{\mu^2 L^2 d^2}{4}, \label{eq: dist_smooth_true} \\
&  \| \nabla f_\mu (\mathbf x)\|_2^2 \leq 2 \| \nabla f(\mathbf x) \|_2^2
    + \frac{\mu^2 L^2 d^2 }{2}. \label{eq: up_grad_fsmooth}
% & \mathbb E_{\mathbf u} \left [
% \| 
% \hat \nabla f(\mathbf x)
% \|_2^2
% \right ] \leq 2 d \| \nabla f(\mathbf x) \|^2 + \frac{\mu^2  L^2 d^2}{2}
% \label{eq: second_moment_grad_random}
\end{align}

 3) For any $\mathbf x \in \mathbb R^d$,
 \begin{align}
  \mathbb E_{\mathbf u} \left [ \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) \|_2^2 
    \right ] \leq 
 \mathbb E_{\mathbf u} \left [
\| 
\hat \nabla f(\mathbf x)
\|_2^2
\right ] \leq 2 d \| \nabla f(\mathbf x) \|_2^2 + \frac{\mu^2  L^2 d^2}{2}.
\label{eq: second_moment_grad_random}
\end{align}
% \begin{align}
%   & \mathbb E_{\mathbf u} \left [ \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) \|^2 
%     \right ]  \leq  \mathbb E_{\mathbf u} \left [
% \| 
% \hat \nabla f(\mathbf x)
% \|_2^2
% \right ] 
% \nonumber \\
% & \leq 
%  2d \| \nabla f(\mathbf x) \|_2^2 + \frac{\mu^2}{2} L^2 d^2.
%  \label{eq: var_grad_est_random}
% \end{align}
\end{mylemma}
\textbf{Proof:}
First, by using \citep[Lemma\,4.1.a]{gao2014information} (also see \citep{shalev2012online} and \citep{nesterov2015random}), we immediately obtain that 
$f_\mu$ is $L_\mu$ smooth with $L_\mu \leq L$, and 
\begin{align}
  \nabla f_\mu (\mathbf x) 
     = \mathbb E_{\mathbf u }
    \left [
    \frac{d}{\mu} f(\mathbf x + \mu \mathbf u) \mathbf u
    \right ].    
\end{align}
Since $\mathbb E_{\mathbf u} [(d/\mu) f(\mathbf x) \mathbf u] = 0 $, we obtain
\eqref{eq: smooth_est_grad}.

% The first equality in \eqref{eq: smooth_est_grad} has been proved by several work, e.g.,
% \citep[Lemma\,4.1.a]{gao2014information}, \citep{shalev2012online} and \citep{nesterov2015random}.
% The second equality in \eqref{eq: smooth_est_grad} holds due to 
% $\mathbb E_{\mathbf u} [(d/\mu) f(\mathbf x) \mathbf u] = 0 $.

Next, we obtain  \eqref{eq: dist_f_smooth_true_random}-\eqref{eq: up_grad_fsmooth} based on \citep[Lemma\,4.1.b]{gao2014information}.
Moreover, we have
\begin{align}
     \| \nabla f_\mu (\mathbf x)\|_2^2 =  &   \| \nabla f_\mu (\mathbf x) - \nabla f (\mathbf x) + \nabla f (\mathbf x)  \|_2^2  \nonumber \\
     \leq & 2   \|  \nabla f (\mathbf x)  \|_2^2  +
     2  \| \nabla f_\mu (\mathbf x) - \nabla f (\mathbf x)   \|_2^2 \nonumber \\
     \overset{\eqref{eq: dist_smooth_true}}{\leq}  &  2 \| \nabla f(\mathbf x) \|_2^2
    + \frac{\mu^2 d^2 L^2}{2},
\end{align}
where the first inequality holds due to Lemma\,\ref{lemma: sum_exp_bd}.


The first inequality of \eqref{eq: second_moment_grad_random}
holds due to \eqref{eq: smooth_est_grad} and  $\mathbb E[\| \mathbf a - \mathbb E[ \mathbf a ]\|_2^2] \leq \mathbb E [\| \mathbf a \|_2^2]$ for a random variable $\mathbf a$. And the second inequality of 
 \eqref{eq: second_moment_grad_random} holds due to  \citep[Lemma\,4.1.b]{gao2014information}.
The proof is now complete. \hfill $\square$


%%%%%%%%%%% average random gradient estimator

In Lemma\,\ref{lemma: smooth_f_random_ave}, we show the properties of   \ref{eq: grad_rand_ave}.

\begin{mylemma}
\label{lemma: smooth_f_random_ave}
%\citep[Lemma\,4.1]{gao2014information}
Following the conditions of Lemma\,\ref{lemma: smooth_f_random}, then   \ref{eq: grad_rand_ave} yields:

1) For any $\mathbf x \in \mathbb R^d$
\begin{align}\label{eq: smooth_est_grad_ave}
    \nabla f_\mu (\mathbf x) = \mathbb E 
    \left [
    \hat \nabla f(\mathbf x)
    \right ],
\end{align}
where $\hat \nabla f(\mathbf x)$ is given by \ref{eq: grad_rand_ave}.


% 2) For any $\mathbf x \in \mathbb R^d$
% \begin{align}
%  \mathbb E_{\mathbf u} \left [
% \| 
% \hat \nabla f(\mathbf x)
% \|_2^2
% \right ] \leq & 2 \left (1 + \frac{d}{q} \right ) \| \nabla f(\mathbf x) \|_2^2  + \left (1+\frac{1}{q} \right ) \frac{\mu^2 L^2 d^2}{2}.
% %2 d \| \nabla f(\mathbf x) \|^2 + \frac{\mu^2}{2} L^2 d^2
% \label{eq: second_moment_grad_random_ave}
% \end{align}

2) For any $\mathbf x \in \mathbb R^d$
\begin{align}
   & \mathbb E \left [ \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) \|_2^2 
    \right ]  \leq  \mathbb E  \left [
\| 
\hat \nabla f(\mathbf x)
\|_2^2
\right ] 
 \leq 2 \left (1 + \frac{d}{q} \right ) \| \nabla f(\mathbf x) \|_2^2 + \left (1+\frac{1}{q} \right ) \frac{\mu^2 L^2 d^2}{2}.
 %2d \| \nabla f(\mathbf x) \|_2^2 + \frac{\mu^2}{2} L^2 d^2.
 \label{eq: var_grad_est_random_ave}
\end{align}
\end{mylemma}
\textbf{Proof}:
Since $\{ \mathbf u_i \}_{i=1}^q$ are i.i.d. random vectors, we have
\begin{align}
    \mathbb E \left [
    \hat \nabla f(\mathbf x)
    \right ] = \mathbb E_{\mathbf u_i} \left [
    \hat \nabla f(\mathbf x; \mathbf u_i)
    \right ] \overset{\eqref{eq: smooth_est_grad}}{=} \nabla f_\mu (\mathbf x),
\end{align}
where 
$
 \hat \nabla f(\mathbf x; \mathbf u_i) \Def
  \frac{d}{\mu} [  f ( \mathbf x + \mu \mathbf u_i ) - f ( \mathbf x  )]  \mathbf u_i
$.

In  \eqref{eq: var_grad_est_random_ave}, the first inequality 
holds due to \eqref{eq: smooth_est_grad_ave} and  $\mathbb E[\| \mathbf a - \mathbb E[ \mathbf a ]\|_2^2] \leq \mathbb E [\| \mathbf a \|_2^2]$ for a random variable $\mathbf a$.
Next, we bound the second moment of $\hat \nabla f(\mathbf x)$
\begin{align}
\mathbb E \left [ \left \| \hat{\nabla} f(\mathbf x) \right  \|_2^2  \right ]  =& \mathbb E \left [ \left  \| \frac{1}{q}\sum_{i=1}^{q}  \left ( \hat \nabla f(\mathbf x; \mathbf u_i)   - {\nabla} f_\mu(\mathbf x)  \right ) + {\nabla} f_\mu(\mathbf x)  \right \|_2^2 \right ] \nonumber \\
= &  \left \| {\nabla} f_\mu(\mathbf x)  \right \|_2^2 + \mathbb E \left [ \left  \| \frac{1}{q }\sum_{i=1}^{q}    \left ( \hat \nabla f(\mathbf x; \mathbf u_i)   - {\nabla} f_\mu(\mathbf x)  \right )  \right \|_2^2 \right ] \nonumber \\
 = &   \left \| {\nabla} f_\mu(\mathbf x)  \right \|_2^2 + \frac{1}{q} 
 \mathbb E \left [ \left  \|  \hat \nabla f(\mathbf x; {\color{black}\mathbf u_1})   - {\nabla} f_\mu(\mathbf x)  \right \|_2^2 \right  ],
% = & \| \bar{\mathbf g} \|^2 + \frac{1}{q} \mathbb E[ \| \hat{\mathbf g}_{1} \|^2 ]  - \frac{1}{q}  \| \bar{\mathbf g} \|^2,
 \label{eq: second_est_ave}
\end{align}
where the expectation is taken with respect to i.i.d. random vectors $\{ \mathbf u_i \}$, and we have used the fact that 
 $\mathbb E[ \|\hat \nabla f(\mathbf x; \mathbf u_i)   - {\nabla} f_\mu(\mathbf x) \|_2^2] = \mathbb E[ \| \hat \nabla f(\mathbf x; \mathbf u_1)   - {\nabla} f_\mu(\mathbf x)  \|_2^2]$ for any $i$. 
 Substituting \eqref{eq: up_grad_fsmooth} and \eqref{eq: second_moment_grad_random} into \eqref{eq: second_est_ave}, we obtain
\eqref{eq: var_grad_est_random_ave}. %{\color{green}using $\mathbf u_1$ is little confusing but it may still be ok}
\hfill $\square$


In Lemma\,\ref{lemma: deter_smooth_gradest}, we demonstrate the properties of   \ref{eq: grad_e}.


    \begin{mylemma}\label{lemma: deter_smooth_gradest}
    Let Assumption A1  hold and define $ f_{\mu_\ell} (\mathbf x) = \mathbb E_{u \sim U [-\mu_\ell, \mu_\ell]} f(\mathbf x + u \mathbf e_\ell)$, where $U [-\mu_\ell, \mu_\ell]$ denotes the uniform distribution at the interval $[-\mu_\ell, \mu_\ell]$. We then have:
    %1) The smoothing function $f_\ell$ is differentiable and $L$-smooth. 
    
    1)  $f_{\mu_\ell}$ is L-smooth, and 
    \begin{align}\label{eq: grad_f_smooth_coord_all}
    { \hat \nabla } f(\mathbf x) = \sum_{\ell = 1}^d  \frac{\partial  f_{\mu_\ell} (\mathbf x) }{\partial x_\ell} \mathbf e_\ell,
\end{align}
where $  { \hat \nabla } f(\mathbf x) $ is defined by \ref{eq: grad_e}, and $\partial f / \partial x_\ell$ denotes the partial derivative with respect to 
      the $\ell$th coordinate.

    
    2) For $\ell \in [d]$,
      \begin{align}
       & |  f_{\mu_\ell} (\mathbf x) - f (\mathbf x)|    \leq \frac{L \mu_\ell^2}{2},
          \label{eq: diff_f_coordinate_abs}
          \\
          & \left | \frac{\partial  f_{\mu_\ell} (\mathbf x) }{\partial x_\ell}   -  \frac{\partial f  (\mathbf x) }{\partial x_\ell} \right | \leq \frac{L \mu_\ell }{2}. \label{eq: diff_grad_coordinate_abs}
    \end{align}
    
    
    3) For $\ell \in [d]$,  
    \begin{align}\label{eq: grad_diff_allcoord}
 \left \| \hat{\nabla} f(\mathbf x) - \nabla f(\mathbf x)  \right \|_2^2 
  \leq \frac{L^2 d}{4} \sum_{\ell = 1}^d \mu_\ell^2.
\end{align}
    % \begin{align}
    %   % & | f_\ell (\mathbf x) - f (\mathbf x)| \leq \frac{L \mu_\ell^2}{2}, \label{eq: f_diff}\\
    %     \left \|  \frac{\partial  f_{\mu_\ell} (\mathbf x) }{\partial x_\ell}   -  \frac{\partial f  (\mathbf x) }{\partial x_\ell}  \right \|_2 \leq \frac{L \mu_\ell }{2}. \label{eq: grad_diff} %\\
    %     % & \mathbb E_\ell \|  \frac{\partial f_\ell (\mathbf x) }{\partial x_\ell}   -  \frac{\partial f  (\mathbf x) }{\partial x_\ell}   \|_2^2\leq \sum_{\ell=1}^d \frac{L^2 \mu_\ell^2}{4d},  \label{eq: sec_grad_diff} 
    % \end{align}
%\textcolor{red}{PY: extra notation $|$ in the LHS of (10)}    
    %where the expectation is taken with respect to the coordinate index $\ell$ which is randomly picked from $[d]$.
    
   %  4) If $f$ is convex, then $f_\ell$ is also convex.
    \end{mylemma}
    \textbf{Proof}: 
  For the $\ell$th coordinate, it is known from \citep[Lemma\,6]{lian2016comprehensive} that $f_{\mu_\ell}$ is $L$-smooth and %{\color{green} equality is only in the limit $\mu_l \xrightarrow{0}$ for next equation right}
  \begin{align}\label{eq: grad_f_smooth_coord}
    \frac{\partial  f_{\mu_\ell} (\mathbf x)}{\partial x_\ell}  = \frac{f( \mathbf x + \mu_{\ell} \mathbf e_\ell ) - f( \mathbf x - \mu_{\ell} \mathbf e_\ell )}{2\mu_\ell}.
    \end{align}
    Based on \eqref{eq: grad_f_smooth_coord} and the definition of \ref{eq: grad_e}, we then obtain \eqref{eq: grad_f_smooth_coord_all}.
    
    The inequalities \eqref{eq: diff_f_coordinate_abs} and \eqref{eq: diff_grad_coordinate_abs}  have   been proved by \citep[Lemma\,6]{lian2016comprehensive}.
    
Based on \eqref{eq: grad_f_smooth_coord_all} and \eqref{eq: diff_grad_coordinate_abs}, we have
    \begin{align}
& \left \| \hat{\nabla} f(\mathbf x) - \nabla f(\mathbf x)  \right \|_2^2 
\overset{\eqref{eq: grad_f_smooth_coord_all}}{=} \left \| \sum_{\ell=1}^d \left ( \frac{\partial  f_{\mu_\ell} (\mathbf x) }{\partial x_\ell} - \frac{\partial f  (\mathbf x)}{\partial x_\ell} \right ) \mathbf e_\ell  \right \|_2^2 \nonumber \\
\leq & d \sum_{\ell=1}^d \left \|  \frac{\partial  f_{\mu_\ell} (\mathbf x) }{\partial x_\ell} - \frac{\partial f  (\mathbf x)}{\partial x_\ell} \right \|_2^2 \leq \frac{L^2 d}{4} \sum_{\ell = 1}^d \mu_\ell^2, \nonumber
\end{align}
where the first inequality holds due to Lemma\,\ref{lemma: sum_exp_bd} in Sec.\,\ref{app: aux}.
The proof is now complete. \hfill $\square$


\subsection{Control variates}\label{supp: control_var}
 The gradient blending   
 in Step\,6 of SVRG (Algorithm\,1) can be interpreted using control variate  \citep{tucker2017rebar,grathwohl2017backpropagation,chatterji2018theory}. If we view $\hat {\mathbf g}_0 \Def \nabla f_{\mathcal I} (\mathbf x)$ as the raw gradient estimate at $\mathbf x$, and    $\mathbf c \Def \nabla f_{\mathcal I}(\hat{\mathbf x})$ as a control variate satisfying 
$
 \mathbb E[\mathbf c]
= \nabla f(\hat{\mathbf x})
$, then the gradient blending \eqref{eq: SVRG_update} becomes a   gradient estimate modified by a  control variate,
$
\hat{\mathbf g} = \hat {\mathbf g}_0 - (\mathbf c - \mathbb E[\mathbf c])
$. 
Here $\hat{\mathbf g}$  has the same expectation as $\hat {\mathbf g}_0$, i.e., $\mathbb E[\hat{\mathbf g}] = \mathbb E[ \hat {\mathbf g}_0 ] = \nabla f(\mathbf x)$, however, has a lower variance when $\mathbf c$ is positively
correlated with $\mathbf g_0$ (see a detailed analysis as below).

Consider the following gradient estimator,
\begin{align}
    \hat{\mathbf g} = \hat {\mathbf g}_0 - \eta (\mathbf c - \mathbb E[\mathbf c]),
\end{align}
where $\hat {\mathbf g}_0$ is a given (raw) gradient estimate, $\eta$ is an unknown coefficient,  and $\mathbf c$ is a control variate. 
It is clear that $ \hat{\mathbf g} $ has the same expectation as $\hat {\mathbf g}_0$. We then study the effect of $\mathbf c$ on the variance of $ \hat{\mathbf g} $,
\begin{align} \label{eq: trace_cov_cv}
   \tr ( \cov(\hat {\mathbf g} ) )  =  \tr( \cov ( {\hat {\mathbf g}_0}) )
    + \eta^2  \tr (\cov( \mathbf  c ) ) - 2 \eta  \tr ( \cov(\hat {\mathbf g}_0,\mathbf c ) ),
\end{align}
where $\tr(\cdot)$ denotes the trace operator, and $\cov(\cdot)$ is the covariance operator. 
When  $
\eta = \frac{\tr (\cov(\hat {\mathbf g}_0,\mathbf c) ) }{\tr (\cov( \mathbf c ))}
%- \mathrm{Cov}(\hat {\mathbf g},\mathbf c_{\boldsymbol \phi} ) \var^{-1}( \mathbf  c_{\boldsymbol \phi} )
$, the  variance of $\hat {\mathbf g}$  in \eqref{eq: trace_cov_cv} is then minimized, leading to
\begin{align}\label{eq: minvar_con}
   & \tr ( \cov(\hat {\mathbf g} )   )  = \tr( \cov (\hat {\mathbf g}_0) ) \left (
   1 - \rho(\hat{\mathbf g}_0, \mathbf c)^2
   \right ),
\end{align}
where
$  \rho(\hat{\mathbf g}_0, \mathbf c) = 
\frac{\tr ( \cov(\hat {\mathbf g}_0,\mathbf c) ) }{ \sqrt{\tr( \cov (\hat {\mathbf g}_0) )} \sqrt{ \tr (\cov(\mathbf  c ))} }
$. In \eqref{eq: minvar_con}, $ \rho(\hat{\mathbf g}_0, \mathbf c)$ indicates  the correlation strength between $\hat{\mathbf g}_0$ and $ \mathbf c$. Therefore, the   gradient estimate $\hat{\mathbf g}$ has a smaller variance than $\hat {\mathbf g}_0$  when the control variate $\mathbf c$ is \textit{positively} correlated with the latter. Moreover, if $\mathbf c$ is chosen  similar to $\hat{\mathbf g}$, then $\eta  $ would be close to 1. 

\subsection{Proof of Proposition~\ref{prop: vks}}\label{supp: lemma_vks}
In  Algorithm\,2, we recall that the mini-batch $\mathcal I$ is chosen uniformly randomly (with  replacement). Based on \eqref{eq: exp_minibatch_2} in Lemma\,\ref{lemma: minibatch}, we have  
\begin{align}\label{eq: E_Iv_v}
    \mathbb E_{\mathcal I_k} [\hat \nabla f_{\mathcal I_k}(\mathbf x_k^s) - \hat \nabla f_{\mathcal I_k}(\mathbf x_0^s)] = \hat \nabla f(\mathbf x_k^s) - \hat \nabla f(\mathbf x_0^s).
    %= \hat \nabla f(\mathbf x_k^s)  + \mathbf e_s.
\end{align}
We   then rewrite $\hat{\mathbf v}_k^s$ as
 \begin{align}\label{eq: E_Iv_v_2}
     \hat {\mathbf v}_k^s = & \hat \nabla f_{\mathcal I_k}(\mathbf x_k^s) - \hat \nabla f_{\mathcal I_k}(\mathbf x_0^s)  -  \mathbb E_{\mathcal I_k} [\hat \nabla f_{\mathcal I_k}(\mathbf x_k^s) - \hat \nabla f_{\mathcal I_k}(\mathbf x_0^s)] +  \hat \nabla f(\mathbf x_k^s).
 \end{align}
% Since  $\mathbb E [ \| \mathbf a - \mathbb E [\mathbf a ] \|_2^2 ] \leq \mathbb E [ \| \mathbf a \|_2^2]$ for a random variable $\mathbf a$, we have
Taking the expectation of $\|  \mathbf v_k^s \|_2^2$ with repsect to all the random variables, we have
 \begin{align}\label{eq: vks_norm_SVRG}
      \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2  \right ]  \leq 
      & 2\mathbb E \left  [ \| \hat \nabla f_{\mathcal I_k}(\mathbf x_k^s) - \hat \nabla f_{\mathcal I_k}(\mathbf x_0^s)  -  \mathbb E_{\mathcal I_k} [\hat \nabla f_{\mathcal I_k}(\mathbf x_k^s) - \hat \nabla f_{\mathcal I_k}(\mathbf x_0^s)]    \|_2^2  \right ]   + 2 \mathbb E \left [\|\hat \nabla f(\mathbf x_k^s) \|_2^2  \right ] \nonumber \\
   \leq &
     \frac{2}{b}  \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s ) -   \mathbb E_{i} [\hat \nabla f_{i}(\mathbf x_k^s) - \hat \nabla f_{i}(\mathbf x_0^s) ]  \|_2^2 \right ] + 2 \mathbb E \left [\|\hat \nabla f(\mathbf x_k^s) \|_2^2  \right ] \nonumber \\
    \leq   &  \frac{2}{b}  \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s ) \|_2^2 \right ] + 4d \mathbb E \left [
    \| \nabla f(\mathbf x_k^s)  \|_2^2 
    \right ] + \mu^2 d^2 L^2,
 \end{align}
 where the  first inequality holds due to Lemma\,\ref{lemma: sum_exp_bd},  the second inequality holds due to Lemma\,\ref{lemma: minibatch}, and the third inequality holds due to $\mathbb E[\| \mathbf a - \mathbb E[ \mathbf a ]\|_2^2] \leq \mathbb E [\| \mathbf a \|_2^2]$ and \eqref{eq: up_grad_fsmooth}.
% and we recall that $\mu$ is a smoothing parameter.
 
 Similar to Lemma\,\ref{lemma: smooth_f_random}, we introduce 
 a smoothing function  $f_{i,\mu}$ of $f_i$, and continue to bound the first term at the right hand side (RHS) of \eqref{eq: vks_norm_SVRG}. This yields
\begin{align}\label{eq: 1st_term_norm_vks}
 & \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s )   \|_2^2 \right ]
 \nonumber \\  \overset{\eqref{eq: sum_exp_bd}}{\leq}   & 3 \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \nabla f_{i,\mu} ( \mathbf x_k^s )\|_2^2 \right ]    + 3 \mathbb E \left [ \|\hat \nabla f_{i,\mu} ( \mathbf x_0^s )
     -   \nabla f_{i} ( \mathbf x_0^s )   \|_2^2 \right  ]  \nonumber \\
     & +       3 \mathbb E \left [ \| \nabla f_{i,\mu} ( \mathbf x_k^s ) -  \nabla f_{i,\mu} ( \mathbf x_0^s ) \|_2^2 \right ] \nonumber \\
     \overset{\eqref{eq: second_moment_grad_random}}{\leq}
     & 6d \mathbb E[ \| \nabla f_{i} (\mathbf x_k^{s}) \|_2^2 ] +  6d \mathbb E[ \| \nabla f_{i} (\mathbf x_0^{s}) \|_2^2 ]   + 3  L^2 d^2 \mu^2 +  3 \mathbb E \left [ \| \nabla f_{i,\mu} ( \mathbf x_k^s ) -  \nabla f_{i,\mu} ( \mathbf x_0^s ) \|_2^2 \right ].
 \end{align}
Since both $f_i$ and $f_{i,\mu}$ are $L$-smooth (A1 and Lemma\,\ref{lemma: smooth_f_random}), we have
\begin{align}
& \mathbb E \left [ \| \nabla f_{i,\mu} ( \mathbf x_k^s ) -  \nabla f_{i,\mu} ( \mathbf x_0^s ) \|_2^2 \right ] \leq  L^2 \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ], \label{eq: vks_bd1} \\
  &  \mathbb E \left [ \| \nabla f_{i} (\mathbf x_0^{s}) \|_2^2 \right ] \leq 
 2 \mathbb E \left [ \| \nabla f_{i} (\mathbf x_0^{s})  - \nabla f_{i} (\mathbf x_k^{s}) \|_2^2  \right ] + 2 \mathbb E \left [\| \nabla f_{i} (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\
& \hspace*{0.9in} \leq  2L^2 \mathbb E \left [ \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2 \right ]+ 2 \mathbb E \left [\| \nabla f_{i} (\mathbf x_k^{s}) \|_2^2 \right ]. %\nonumber \\
 %\leq &  2L^2 \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2+ 4  \mathbb E \left [  \| \nabla f_{i} (\mathbf x_k^{s}) - \nabla f (\mathbf x_k^{s})  \|_2^2 \right ]  + 4 \mathbb E \left [\| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ]  \nonumber \\
 %\leq &  2L^2 \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2+ 4\sigma^2 + 4 \mathbb E \left [\| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ],
 \label{eq: vks_bd2}
\end{align}
%where the last inequality holds due to Assumption A2. 
 Substituting \eqref{eq: vks_bd1} and \eqref{eq: vks_bd2} into \eqref{eq: 1st_term_norm_vks}, we obtain
 \begin{align}\label{eq: 1st_term_norm_vks_2}
  &   \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s )   \|_2^2 \right ] \nonumber \\
     \leq & 18d \mathbb E[ \| \nabla f_{i} (\mathbf x_k^{s}) \|_2^2 ] +  (12d+3)L^2  \mathbb E \left [ \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2 \right ] + 3  L^2 d^2 \mu^2 \nonumber \\
     \leq & 36d \mathbb E \left [  \| \nabla f_{i} (\mathbf x_k^{s}) - \nabla f (\mathbf x_k^{s})  \|_2^2 \right ]  + 36d \mathbb E \left [\| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\
     & + (12d+3)L^2  \mathbb E \left [ \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2 \right ] + 3  L^2 d^2 \mu^2 \nonumber \\
     \leq & 36 d \sigma^2 + 36d \mathbb E \left [\| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] + (12d+3)L^2  \mathbb E \left [ \| \mathbf x_0^{s} - \mathbf x_k^{s} \|_2^2 \right ] + 3  L^2 d^2 \mu^2,
 \end{align}
where the last inequality holds due to Assumption A2. 

Substituting \eqref{eq: 1st_term_norm_vks_2} into \eqref{eq: vks_norm_SVRG}, we then complete the proof.
\hfill $\square$

 
 
 \subsection{Proof of Theorem~\ref{thr: ZO_SVRG_rand}}\label{supp: thr1}
Since  $f_\mu$ is $L$-smooth (Lemma\,\ref{lemma: smooth_f_random}), from    Lemma\,\ref{lemma: Lsmooth_v2} in Sec.\,\ref{app: aux} we have 
\begin{align}\label{eq: fsmooth_def_SVRG}
f_{\mu} (\mathbf x_{k+1}^s) \leq & f_{\mu} (\mathbf x_k^s) +  \inp{\nabla f_{\mu} (\mathbf x_k^s)  }{\mathbf x_{k+1}^s - \mathbf x_k^s}  + \frac{L}{2} \| x_{k+1}^s - \mathbf x_k^s \|_2^2 \nonumber \\
= &  f_{\mu} (\mathbf x_k^s) -  \eta_k \inp{\nabla f_{\mu} (\mathbf x_k^s)  }{\hat {\mathbf v}_k^s}  + \frac{L}{2} \eta_k^2 \| \hat {\mathbf v}_k^s \|_2^2,
\end{align}
where the last equality holds due to $\mathbf x_{k+1}^{s} = \mathbf  x_{k}^{s} - \eta_{k} \hat {\mathbf v}_{k}^{s}$.
Since $\mathbf x_{k}^s$ and $\mathbf x_0^s$  are independent of $\mathcal I_{k}$ and   random directions $\mathbf u$ used for ZO gradient estimates, from \eqref{eq: smooth_est_grad} and \eqref{eq: exp_minibatch_2} (Lemma\,\ref{lemma: minibatch}) we obtain
\begin{align}\label{eq: E_uIk_v}
    \mathbb E_{\mathbf u, \mathcal I_{k}} \left [\hat {\mathbf v}_{k}^s \right ]   = & \mathbb E_{\mathbf u, \mathcal I_{k}} \left [ \hat{\nabla} f_{{\mathcal I}_{k}} ( {\mathbf x}_{k}^{s}) - \hat{\nabla} f_{{\mathcal I}_{k}} ( {\mathbf x}_{0}^{s}) + \hat{\nabla} f (\mathbf x_0^s) \right ] \nonumber \\
    = &  \nabla f_\mu(\mathbf x_{k}^s)  + \nabla  f_{\mu} (\mathbf x_0^s) - \nabla f_\mu (\mathbf x_0^s)     =  \nabla f_\mu(\mathbf x_{k}^s).
\end{align}
Combining \eqref{eq: fsmooth_def_SVRG} and \eqref{eq: E_uIk_v}, we have
\begin{align}\label{eq: fsmooth_def_SVRG2}
 \mathbb E \left [ f_{\mu} (\mathbf x_{k+1}^s) \right ] \leq & \mathbb E \left [ f_{\mu} (\mathbf x_k^s) \right ] - \eta_k \mathbb E \left [ \| \nabla f_\mu(\mathbf x_{k}^s) \|_2^2 \right ]  + \frac{L}{2} \eta_k^2 \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ],   
\end{align}
where the expectation is taken with respect to all random variables. 
 
 At RHS of \eqref{eq: fsmooth_def_SVRG2}, the upper bound on $\mathbb E \left [ \| \mathbf v_k^s \|_2^2 \right ]$ is given by %\eqref{eq: vks_norm_SVRG2} in
 Proposition\,\ref{prop: vks},
\begin{align}
\label{eq: vks_norm_SVRG2_v2}
    \mathbb E[ \| \hat{ \mathbf v}_{k}^s \|_2^2]  \leq &
  \frac{4(b+18)d}{b}  \mathbb E\left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2  \right ]+ \frac{6(4d+1)L^2}{b} \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
  &+ \frac{  (6 +b)  L^2 d^2 \mu^2}{b} + \frac{ 72d \sigma^2}{b}.
\end{align} 
In \eqref{eq: vks_norm_SVRG2_v2}, we   further bound $\mathbb E \left [\| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2 \right ]$ as
\begin{align}\label{eq: norm_xk_dif}
  & \mathbb E \left [\| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2 \right ] 
  =   \mathbb E \left [\| \mathbf x_{k+1}^s -\mathbf x_{k}^s + \mathbf x_{k}^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
  = & 
   \eta_k^2 \mathbb E \left [
   \| \hat {\mathbf v}_{k}^s\|_2^2
   \right ] + \mathbb E \left [
   \|
  \mathbf x_{k}^s - \mathbf x_0^s
  \|_2^2
   \right ]
  - 2\eta_k  \mathbb E \left [ \inp{\hat {\mathbf v}_{k}^s}{\mathbf x_{k}^s - \mathbf x_0^s}
  \right ] \nonumber \\
  \overset{\eqref{eq: E_uIk_v}}{=} & \eta_k^2 \mathbb E \left [
   \| \hat {\mathbf v}_{k}^s\|_2^2
   \right ] + \mathbb E \left [
   \|
  \mathbf x_{k}^s - \mathbf x_0^s
  \|_2^2
   \right ]
  - 2\eta_k  \mathbb E \left [ \inp{\nabla f_\mu(\mathbf x_k^s)}{\mathbf x_{k}^s - \mathbf x_0^s}
  \right ] \nonumber \\
  \leq & \eta_k^2 \mathbb E \left [
   \| \hat {\mathbf v}_{k}^s\|_2^2
   \right ] + \mathbb E \left [
   \|
  \mathbf x_{k}^s - \mathbf x_0^s
  \|_2^2
   \right ]
   + 2 \eta_k\mathbb E \left [
  \frac{1}{2\beta_k}   \| \nabla f_\mu(\mathbf x_{k}^s) \|_2^2 + \frac{\beta_k}{2}  \| \mathbf x_{k}^s - \mathbf x_0^s \|_2^2
  \right ],
\end{align}
where $\beta_k $ is a positive coefficient, and the last inequality holds since $\inp{\mathbf a}{\mathbf b} \leq \frac{\beta \| \mathbf a \|_2^2 + (1/\beta) \| \mathbf b \|_2^2}{2}$ for any $\mathbf a$ and $\mathbf b$, and $\beta > 0$.

Now with \eqref{eq: vks_norm_SVRG2_v2} and \eqref{eq: norm_xk_dif} at hand, we introduce 
a   Lyapunov function  \citep{reddi2016stochastic} with respect to $f_\mu$,
\begin{align}\label{eq: Def_Rks}
    R_{k}^s = \mathbb E \left [ f_\mu (\mathbf x_k^s) + c_k \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ],
\end{align}
for some $c_k > 0 $.
Substituting \eqref{eq: fsmooth_def_SVRG2} and \eqref{eq: Def_Rks} into $R_{k+1}^s$, we obtain
\begin{align}
\label{eq: Rk_new_SCRG}
   R_{k+1}^s 
    =  & \mathbb E \left [ f_\mu (\mathbf x_{k+1}^s) + c_{k+1} \| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
    \leq & \mathbb E \left [f_{\mu} (\mathbf x_k^s) - \eta_k \| \nabla f_{\mu} (\mathbf x_k^s)  \|_2^2 + \frac{L}{2} \eta_k^2 \| \hat {\mathbf v}_k^s \|_2^2 \right ] \nonumber \\
    & + \mathbb E \left [
    c_{k+1} \eta_k^2 \| \hat {\mathbf v}_k^s \|_2^2 + c_{k+1} \| \mathbf x_k^s - \mathbf x_0^s \|_2^s
    \right ] \nonumber \\
    & + \mathbb E \left [ \frac{c_{k+1} \eta_k}{\beta_k} \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 + c_{k+1} \beta_k \eta_k \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ] \nonumber\\
    = & \mathbb E \left [ f_\mu (\mathbf x_k^s) \right ] - \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 \right ] \nonumber \\
   & + \left (c_{k+1} + c_{k+1} \beta_k \eta_k \right ) \mathbb E \left [ \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ]  + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2  \right ) \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ].
\end{align}
Moreover, substituting \eqref{eq: vks_norm_SVRG2_v2} into \eqref{eq: Rk_new_SCRG}, we have
\begin{align}
\label{eq: Rk_new_SCRG_2}
  R_{k+1}^s  
  \leq &   \mathbb E \left [ f_\mu (\mathbf x_k^s) \right ] - \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 \right ]   + \left (c_{k+1} + c_{k+1} \beta_k \eta_k \right ) \mathbb E \left [ \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{6(4d+1)L^2}{b} \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{4db + 72d }{b } \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b) L^2 d^2 \mu^2 + 72d \sigma^2 }{b}.
\end{align}
Based on the definition of $
    c_k = c_{k+1} + \beta_k \eta_k  c_{k+1} + \frac{6 (4d+1)  L^2 \eta_k^2}{b} c_{k+1} + \frac{3 (4d+1) L^3 \eta_k^2}{b}
$ and the definition of $R_k^s$ in \eqref{eq: Def_Rks}, we can simplify the inequality \eqref{eq: Rk_new_SCRG_2} as
\begin{align}
\label{eq: Rk_new_SCRG_2_2}
 R_{k+1}^s  
  \leq &  R_k^s - \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 \right ]     + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{4db + 72d }{b } \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b) L^2 d^2 \mu^2 + 72d \sigma^2 }{b} \nonumber \\
\overset{\eqref{eq: up_grad_fsmooth}}{\leq } & R_k^s - \frac{1}{2} \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f(\mathbf x_k^s) \|_2^2 \right ]   
+ \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \frac{\mu^2 d^2 L^2}{4} \nonumber \\
& + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{4db + 72d }{b } \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b) L^2 d^2 \mu^2 + 72d \sigma^2 }{b} \nonumber \\
= & R_k^s  - \gamma_k \mathbb E \left [ \| \nabla f(\mathbf x_k^s) \|_2^2 \right ]   
+ \chi_k,
\end{align}
where $\gamma_k$ and $\chi_k$ are coefficients given by
\begin{align}
&    \gamma_k = \frac{1}{2} \left (1-  \frac{c_{k+1} }{\beta_k} \right ) \eta_k
    - \left ( \frac{L}{2} + c_{k+1} \right ) \frac{4db + 72d }{b } \eta_k^2,\\
    & 
    \chi_k = \left ( \frac{L}{2}  + c_{k+1} \right )\frac{ (6+b) L^2 d^2 \mu^2 + 72d \sigma^2 }{b}\eta_k^2 + \left (1-  \frac{c_{k+1} }{\beta_k} \right ) \frac{\mu^2 d^2 L^2}{4}\eta_k.
\end{align}


Taking a telescopic sum for \eqref{eq: Rk_new_SCRG_2_2}, we obtain 
\begin{align}\label{eq: Rk_new_SCRG_4}
    R_m^s \leq & R_0^s - \sum_{k=0}^{m-1} \gamma_k \mathbb E \left [\| \nabla f(\mathbf x_k^s) \|_2^2 \right ]   + \chi_m,
\end{align}
where  $\chi_m = \sum_{k=0}^{m-1} \chi_k$.
It is known from \eqref{eq: Def_Rks} that 
\begin{align}
    R_0^s = \mathbb E \left [f_{\mu} (\mathbf x_0^s) \right ], \quad
    R_m^s =  \mathbb E \left [f_{\mu} (\mathbf x_m^s) \right ],
\end{align}
where the last equality used the fact that $c_m = 0$. 
Since $\tilde{\mathbf x}_{s-1} = \mathbf x_0^s $ and $\tilde{\mathbf x}_s = \mathbf x_m^s$, we obtain
\begin{align}\label{eq: R0m_SVRG}
    R_0^s - R_m^s = & \mathbb E \left [f_\mu(\tilde {\mathbf x}_{s-1}) - f_\mu(\tilde {\mathbf x}_s ) \right ]. %\nonumber %\\
   % \leq & \mathbb E[  f(\tilde {\mathbf x}_{s-1}) - f(\tilde {\mathbf x}_s ) ] + L\mu^2,
\end{align}
Substituting \eqref{eq: R0m_SVRG} into \eqref{eq: Rk_new_SCRG_4} and telescoping the sum for $s = 1,2,\ldots,S$, we obtain 
\begin{align}\label{eq: grad_mid_Sm}
     \sum_{s=1}^S \sum_{k=0}^{m-1}\gamma_k  \mathbb E[\| \nabla f(\mathbf x_k^s) \|_2^2]  % \nonumber \\
    \leq    \mathbb E[  f_\mu(\tilde {\mathbf x}_{0}) - f_\mu(\tilde {\mathbf x}_S ) ]  + S \chi_m.
   % \leq  \mathbb E[  f_\mu(\tilde {\mathbf x}_{0}) - f_\mu^* ]  + S \chi_m  
%    \leq  \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ] + L\mu^2 + S \chi_m,
\end{align}
Denoting $f_{\mu}^* = \min_{\mathbf x} f_\mu (\mathbf x)$, from \eqref{eq: smooth_est_grad} we have $f_\mu(\tilde {\mathbf x}_{0}) - f(\tilde {\mathbf x}_{0}) \leq \frac{\mu^2 L}{2}$ and $f^* - f_\mu^* \leq  \frac{\mu^2 L}{2}$, where $f^* =  \min_{\mathbf x} f (\mathbf x)$. This yields
 \begin{align}\label{eq: dist_func_random_grad}
  f_\mu(\tilde {\mathbf x}_{0}) - f_\mu(\tilde {\mathbf x}_S ) \leq 
  f_\mu(\tilde {\mathbf x}_{0}) - f_\mu^* \leq ( f(\tilde {\mathbf x}_{0}) - f^* )
   + \mu^2 L.
\end{align}
Substituting \eqref{eq: dist_func_random_grad} into \eqref{eq: grad_mid_Sm}, we have
\begin{align}\label{eq: grad_mid_Sm_v2}
   \sum_{s=1}^S \sum_{k=0}^{m-1}\gamma_k  \mathbb E[\| \nabla f(\mathbf x_k^s) \|_2^2]  % \nonumber \\
    \leq    \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ] + L \mu^2 + S \chi_m.
\end{align}

Let $\bar{\gamma} = \min_k \gamma_k$ and we choose
 $\bar{\mathbf x}$  uniformly random from $\{ \{ {\mathbf x}_k^s \}_{k=0}^{m-1} \}_{s=1}^S$, then ZO-SVRG satisfies
\begin{align}\label{eq: conv_SVRG_0}
       \mathbb E[\| \nabla f(\bar {\mathbf x}) \|_2^2]  
    \leq     \frac{ \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ] }{T \bar \gamma} + \frac{L\mu^2}{T \bar \gamma} + \frac{S \chi_m}{T \bar \gamma}.
\end{align}
The proof is now complete.
\hfill $\square$

\subsection{Proof of Corollary~\ref{col: SVRG_simple}}\label{supp: cor1}
We start by rewriting $c_k$ in \eqref{eq: ck_coeff} as
\begin{align}\label{eq: ck_recursion}
    c_k =  (1+ \theta) c_{k+1}  + \frac{3 (1+4d)L^3 \eta^2}{b},
\end{align}
where $\theta = \beta \eta + \frac{6(1+4d)L^2  \eta^2}{b}$. The recursive formula   \eqref{eq: ck_recursion} implies that $c_k \leq c_0$ for any $k$, and
\begin{align}\label{eq: c0}
    c_0  = \frac{3 (1+4d) L^3 \eta^2}{b} \frac{(1+ \theta)^m - 1}{\theta}.
\end{align}
Based on the choice of $\eta = \frac{\rho}{L d}$ and $\beta = L$, we have 
\begin{align}\label{eq: theta}
    \theta = \frac{\rho}{ d} + \frac{6  \rho^2 }{ b  d^2}  + \frac{24  \rho^2 }{  b d} \leq \frac{31 \rho}{ d}.
\end{align}
Substituting \eqref{eq: theta} into \eqref{eq: c0}, we have
\begin{align}\label{eq: ck_upper}
   c_k \leq c_0 & = \frac{3 (1+4d) L^3}{b} \frac{\eta^2}{\theta } [(1+ \theta)^m - 1]   = \frac{3(1+4d)L\rho}{db + 24\rho d + 6\rho}  [(1+ \theta)^m - 1] \nonumber \\
   & \leq \frac{15 d  L \rho }{db}[(1+ \theta)^m - 1]   \leq \frac{15 L \rho}{b} (e - 1) \leq \frac{30L\rho}{b},
 \end{align}
 where the third inequality holds since
 $
 (1+\theta)^m \leq (1+ \frac{31\rho}{d})^m
 $, $m = \ceil{ \frac{d}{31 \rho} } $,   
 $(1 + 1/a)^a \leq   \lim_{a \to \infty} (1 + \frac{1}{a})^a = e
 $ for $a > 0$ \cite[Appendix\,E]{reddi2016stochastic}, and for east of representation, the last inequality   loosely uses the notion `$\leq$' since $e < 3$.
 
  We recall from \eqref{eq: grad_norm_SVRG} and \eqref{eq: coeff_gammak} that
 \begin{align}
     \bar \gamma = \min_{0 \leq k \leq m-1}  \left \{ 
     \frac{\eta_k}{2} - \frac{c_{k+1} \eta_k}{2 \beta_k} 
     - \eta_k^2 \left (\frac{L}{2} + c_{k+1} \right ) \left ( 4d + \frac{72d }{b} \right ) \right \}.
 \end{align}
Since $\eta_k =\eta $, $\beta_k = \beta$, and $c_k \leq c_0$, we have
 \begin{align}\label{eq: min_gam}
     \bar \gamma \geq \frac{\eta}{2} - \frac{c_0}{2 \beta} \eta - \eta^2 L \left (2d + \frac{36d}{b} \right ) - \eta^2 c_0 \left (4d + \frac{72d}{b} \right ).
 \end{align}
 From \eqref{eq: ck_upper} and the definition of $\beta$, we have
 \begin{align}
   &  \frac{c_0}{2\beta} \leq \frac{15\rho}{b} \label{eq: c0_beta} \\
   &  \eta L \left (2d + \frac{36d}{b} \right ) =
     \rho \left (2 + \frac{36}{b} \right )   \label{eq: eta_L} \\
     &   \eta c_0 \left  (4d + \frac{72d}{b} \right ) \leq  
     \frac{\rho}{L d}\frac{30 L \rho}{b } \left  (4d + \frac{72d}{b} \right ) 
    \leq  \frac{120 \rho^2  }{b} +
    \frac{2160 \rho^2  }{b^2}. \label{eq: eta_c0}
 \end{align}
  
 %When $b \geq 18$, 
 Substituting \eqref{eq: c0_beta}-\eqref{eq: eta_c0} into \eqref{eq: min_gam}, we obtain
  \begin{align}
     \bar \gamma \geq & \eta \left (
     \frac{1}{2} - \frac{15 \rho}{b}
   - 4 \rho - \frac{240 \rho^2}{b}
     \right ) 
     \geq 
     \eta \left (
     \frac{1}{2} -
   259 \rho
     \right ), % \nonumber \\
   %  \geq &  \eta \left (
    % \frac{1}{2} -
    % 15c - \frac{244cb}{d^{\frac{2}{3}}}
    % \right ) 
 \end{align}
 where  we have used the fact that
$\rho^2 \leq \rho$. Moreover, if we set $\rho \leq \frac{1}{518}$, then $\bar{\gamma} > 0$. In other words,  the current parameter setting is valid for Theorem\,\ref{thr: ZO_SVRG_rand}.
Upon defining a universal constant $ \alpha_0 =  \left (
     \frac{1}{2} -
   259 \rho
     \right )$, 
we have
\begin{align}\label{eq: gamma_bar_bound}
     \bar \gamma \geq & 
      \eta \alpha_0.
 \end{align}
% where $\alpha_0 > 0$   is independent of $T$, $d$ and $b$.

 Next, we find the upper bound on $\chi_m$ in \eqref{eq: coeff_chik} given the current parameter setting and $c_k \leq c_0$,
 \begin{align}
     \chi_m \leq  m \eta \frac{\mu^2 d^2 L^2}{4}  + m \eta^2 \left ( \frac{L}{2}  + c_{0} \right )\frac{ (6+b) L^2 d^2 \mu^2 + 72d \sigma^2 }{b}.
 \end{align}
 Since 
 $
 \frac{L}{2} + c_0 \leq \frac{L}{2} + 30 L \rho b^{-1} \leq \frac{L}{2} + 2 L = \frac{5 L}{2}
 $ (suppose $b \geq 18$ without loss of generality), based on \eqref{eq: gamma_bar_bound} we have
 \begin{align}
     \frac{\chi_m}{\bar \gamma} \leq&
   m  \frac{d^2 L^2 \mu^2}{4 \alpha_0}  +
    m  \frac{5 L}{2 \alpha_0} \frac{72 d \sigma^2}{b} \frac{\rho}{L d}   + m \frac{5L}{2 \alpha_0} \left (
\frac{6L^2 d^2 \mu^2}{b} + L^2 d^2 \mu^2
\right )\frac{\rho}{L d}.
 \end{align}
 Since  $T = S m$, and  $\mu = \frac{1}{\sqrt{d T}}$, the above inequality yields
 \begin{align}\label{eq: const_error_bd}
     \frac{S\chi_m}{ T \bar \gamma} \leq&
    \frac{d L^2}{4 \alpha_0 T }  +
     \frac{180 \sigma^2 \rho }{b \alpha_0}  +  \frac{5 L^2}{2 \alpha_0} \left (
\frac{6  }{b} +  1
\right )  \frac{\rho}{  T} 
=  O \left (
\frac{d}{T} + \frac{1}{b}
\right ),
 \end{align}
 where in the big $O$ notation, we only keep the dominant terms and ignore the constant numbers that are independent of  $d$, $b$, and $T$.
 
  Substituting \eqref{eq: gamma_bar_bound} and 
 \eqref{eq: const_error_bd} into \eqref{eq: grad_norm_SVRG}, we have
\begin{align} \label{eq: grad_norm_SVRG_special}
    \mathbb E[ \| \nabla f(\bar { \mathbf x }) \|_2^2 ] \leq &
\frac{[f(\tilde{\mathbf x}_0) - f^*]}{T \alpha_0 }
\frac{L d}{ \rho }
+   \frac{L^2 }{T^2 \alpha_0 \rho}
+ \frac{S\chi_m}{ T \bar \gamma}  
=  O \left (
\frac{d}{T} + \frac{1}{b}
\right ).
\end{align}


 The proof is now complete. 
 \hfill $\square$
 
 
 
 
 
 
 
 
  \subsection{Proof of Proposition~\ref{prop: grad_err}}\label{supp: grad_err}

For  \ref{eq: grad_rand}, based on \eqref{eq: dist_smooth_true} and \eqref{eq: second_moment_grad_random}, we have
\begin{align}\label{eq: diff_grad_estg}
&     \mathbb E \left [
    \| \hat \nabla f(\mathbf x) - \nabla f(\mathbf x) \|_2^2
    \right ] 
\leq   \mathbb E \left [
    \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) 
    + \nabla f_\mu(\mathbf x)
    - \nabla f(\mathbf x) \|_2^2
    \right ] \nonumber \\
    \leq & 2 \mathbb E \left [  \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) \|_2^2 \right ] + 2  \| \nabla f_\mu(\mathbf x)
    - \nabla f(\mathbf x) \|_2^2 \nonumber \\
    \leq & 4d \| \nabla f(\mathbf x) \|_2^2  + \frac{3\mu^2  L^2 d^2}{2}
    = O \left (d \| \nabla f(\mathbf x) \|_2^2 + \mu^2  L^2 d^2
    \right ).
     %\nonumber \\
  %  \leq & 4d \sigma + \frac{3\mu^2 d^2 L^2}{2}.
\end{align}
 

Similarly, for    \ref{eq: grad_rand_ave}, based on \eqref{eq: dist_smooth_true} and \eqref{eq: var_grad_est_random_ave}, we have 
\begin{align}\label{eq: diff_grad_estg_ave}
     \mathbb E \left [
    \| \hat \nabla f(\mathbf x) - \nabla f(\mathbf x) \|_2^2
    \right ] 
% \leq   \mathbb E \left [
%     \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) 
%     + \nabla f_\mu(\mathbf x)
%     - \nabla f(\mathbf x) \|_2^2
%     \right ] \nonumber \\
%     \leq & 2 \mathbb E \left [  \| \hat \nabla f(\mathbf x) - \nabla f_\mu (\mathbf x) \|_2^2 \right ] + 2  \| \nabla f_\mu(\mathbf x)
%     - \nabla f(\mathbf x) \|_2^2
    \leq &  4 \left (1 + \frac{d}{q} \right ) \| \nabla f(\mathbf x) \|_2^2 + \left (3+\frac{2}{q} \right ) \frac{\mu^2 L^2 d^2}{2} \nonumber \\
    = & O \left (
    \frac{q+d}{q} \| \nabla f(\mathbf x) \|_2^2 + \mu^2 L^2 d^2
    \right ),
  %  \leq & 4d \sigma + \frac{3\mu^2 d^2 L^2}{2}.
\end{align}
where we have used the fact that $\frac{2}{q} \leq 3$.

Finally,    using \eqref{eq: grad_diff_allcoord}, the proof is then complete. 
\hfill $\square$
 
 
 
 \subsection{Proof of Theorem~\ref{thr: ZO_SVRG_rand_ave}} \label{supp: thr2}
 
 Motivated by Proposition\,\ref{prop: vks}, we first bound $\| \hat {\mathbf v}_k^s \|_2^2$. Following \eqref{eq: E_Iv_v}-\eqref{eq: vks_norm_SVRG}, we have
 \begin{align}\label{eq: vks_norm_SVRG_ave}
      \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ]  \leq 
      & \frac{2}{b} \mathbb E \left [ \| \hat \nabla f_{i}(\mathbf x_k^s) - \hat \nabla f_{i}(\mathbf x_0^s)  \|_2^2 \right ]   + 2 \mathbb E \left [\|\hat \nabla f(\mathbf x_k^s) \|_2^2  \right ] \nonumber \\
     \overset{\eqref{eq: var_grad_est_random_ave}}{\leq} &
     \frac{2}{b}  \mathbb E [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s )   \|_2^2 ]   + 
    4 \left (1 + \frac{d}{q} \right ) \| \nabla f(\mathbf x) \|_2^2 + \left (1+\frac{1}{q} \right )  \mu^2 L^2 d^2.
 \end{align}
 Moreover, following \eqref{eq: 1st_term_norm_vks}-\eqref{eq: 1st_term_norm_vks_2} together with \eqref{eq: var_grad_est_random_ave}, we can obtain that
 \begin{align}\label{eq: 1st_term_norm_vks_2_ave}
   & \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s ) \|_2^2 \right  ]   \nonumber \\
     \leq &  36 \left (1+\frac{d}{q} \right ) \sigma^2 + 36 \left (1+ \frac{d}{q} \right ) \mathbb E \left [ \| \nabla f (\mathbf x_k^{s}) \|_2^2 \right ]    + \left (12 \frac{d}{q}+15 \right ) L^2 \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \nonumber \\
     & + 3 \left (1+\frac{1}{q} \right ) L^2  \mu^2 d^2.
 \end{align}
 Substituting \eqref{eq: 1st_term_norm_vks_2_ave} into \eqref{eq: vks_norm_SVRG_ave}, we have
 \begin{align}
\label{eq: vks_norm_SVRG2_ave}
    \mathbb E \left [ \| \hat {\mathbf v}_{k}^s \|_2^2 \right ]  
    \leq & 
   \frac{4(b+18)}{b} \left (1+\frac{d}{q} \right )\mathbb E[ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 ]  + \frac{6}{b}\left (\frac{4d}{q}+5 \right )L^2 \| \mathbf x_k^s - \mathbf x_0^s \|_2^2  \nonumber \\
    & + 
    \frac{6+b}{b} \left (1+\frac{1}{q} \right ) L^2 \mu^2 d^2  + \frac{72}{b} \left (1+\frac{d}{q} \right ) \sigma^2.
\end{align}
 
 
 Next, we bound $\mathbb E[\| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2]$.  
 Following \eqref{eq: Def_Rks}-\eqref{eq: Rk_new_SCRG} and substituting \eqref{eq: vks_norm_SVRG2_ave}  into \eqref{eq: Rk_new_SCRG}, we have
 \begin{align}
\label{eq: Rk_new_SCRG_2_ave}
  R_{k+1}^s  
  \leq &   \mathbb E \left [ f_\mu (\mathbf x_k^s) \right ] - \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 \right ]   + \left (c_{k+1} + c_{k+1} \beta_k \eta_k \right ) \mathbb E \left [ \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{6(4d+5q)L^2}{bq} \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{(72 + 4b) (q+d) }{b q} \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& +  \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b)(q+1) L^2 d^2 \mu^2 + 72 (q+d) \sigma^2 }{bq}.
\end{align}
Based on 
%$c_k = c_{k+1} + c_{k+1} \beta_k \eta_k+ \frac{6(4d+5q)L^2}{bq} \eta_k^2 c_{k+1} + 
%\frac{3(4d+5q)L^3}{bq} \eta_k^2$ and 
the definitions of $c_k$  and $R_k^s$  \eqref{eq: Def_Rks}, we can simplify \eqref{eq: Rk_new_SCRG_2_ave} to
\begin{align}
\label{eq: Rk_new_SCRG_2_2_ave}
 R_{k+1}^s  
%   \leq &  R_k^s - \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f_\mu (\mathbf x_k^s) \|_2^2 \right ]    \nonumber \\
%   & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{(72 + 4b)(q+d) }{b q } \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
% & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b)(q+1) L^2 d^2 \mu^2 + 72 (q+d) \sigma^2 }{bq} \nonumber \\
\overset{\eqref{eq: up_grad_fsmooth}}{\leq } & R_k^s - \frac{1}{2} \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \mathbb E \left [ \| \nabla f(\mathbf x_k^s) \|_2^2 \right ]   
+ \left (\eta_k-  \frac{c_{k+1} \eta_k}{\beta_k} \right ) \frac{\mu^2 d^2 L^2}{4} \nonumber \\
& + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \frac{(72 + 4b)(q+d) }{b q } \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{ (6+b)(q+1) L^2 d^2 \mu^2 + 72 (q+d) \sigma^2 }{bq} \nonumber \\
= & R_k^s  - \gamma_k \mathbb E \left [ \| \nabla f(\mathbf x_k^s) \|_2^2 \right ]   
+ \chi_k,
\end{align}
where $ \gamma_k$ and $\chi_k $ are defined coefficients in Theorem\,\ref{thr: ZO_SVRG_rand_ave}.
% \begin{align}
% &    \gamma_k = \frac{1}{2} \left (1-  \frac{c_{k+1} }{\beta_k} \right ) \eta_k
%     - \left ( \frac{L}{2} + c_{k+1} \right ) \frac{(72 + 4b)(q+d) }{b q } \eta_k^2,\\
%     & 
%     \chi_k = \left ( \frac{L}{2}  + c_{k+1} \right )\frac{ (6+b)(q+1) L^2 d^2 \mu^2 + 72 (q+d) \sigma^2 }{bq}\eta_k^2 + \left (1-  \frac{c_{k+1} }{\beta_k} \right ) \frac{\mu^2 d^2 L^2}{4}\eta_k.
% \end{align}

Based on \eqref{eq: Rk_new_SCRG_2_2_ave}
and following the same argument in \eqref{eq: Rk_new_SCRG_4}-\eqref{eq: conv_SVRG_0}, we then achieve
\begin{align} 
       \mathbb E[\| \nabla f(\bar {\mathbf x}) \|_2^2]  
    \leq     \frac{ \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ] }{T \bar \gamma} + \frac{L\mu^2}{T \bar \gamma} + \frac{S \chi_m}{T \bar \gamma}. \label{eq: conv_SVRG_0_ave}
\end{align}


The rest of the proofs essentially follow along the lines of Corollary\,\ref{col: SVRG_simple} with the added complexity of the mini-batch parameter $q$
in $c_k$, $\gamma_k$ and $\chi_k$.

Let $\theta = \beta_k \eta_k+ \frac{6(4d+5q)L^2}{bq} \eta_k^2$, then $c_k = c_{k+1} (1+ \theta)  + \frac{3 (4d+5q) L^3 \eta^2}{bq} $.
This leads to
\begin{align}\label{eq: c0_ave}
    c_0 & = \frac{3 (4d+5q) L^3 \eta^2}{bq} \frac{(1+ \theta)^m - 1}{\theta}.
\end{align}
Based on the choice of $\eta$ and $\beta$, we have 
\begin{align}\label{eq: theta_ave}
    \theta = \frac{\rho}{ d} + \frac{24  \rho^2 }{ b  dq}  + \frac{30  \rho^2 }{  b d^2} \leq \frac{55 \rho}{d}. %\leq \frac{31 b c}{ d}.
\end{align}
Substituting \eqref{eq: theta_ave} into \eqref{eq: c0_ave}, we have
\begin{align}\label{eq: ck_upper_ave}
   c_k \leq c_0 & = \frac{3 (5+4d/q) L^3}{b} \frac{\eta^2}{\theta } [(1+ \theta)^m - 1]   = \frac{3(5+4d/q)L\rho}{db + 24\rho d/q + 30\rho}  [(1+ \theta)^m - 1] \nonumber \\
   & \leq \frac{3(5+4d/q)L\rho}{db}[(1+ \theta)^m - 1]  \leq  \frac{27 L \rho}{b\min\{d,q\}} [(1+ \theta)^m - 1] \nonumber \\
   & \leq \frac{27 L \rho}{b\min\{d,q\}} (e - 1) \leq \frac{54L\rho}{b \min \{ d,q\}},
 \end{align}
 where the third inequality holds since  $5+4d/q \leq 9 d /q$ if $d \geq q$, and $5+4d/q \leq 9 $ otherwise, and the forth inequality holds similar to  \eqref{eq: ck_upper} under $m = \ceil{\frac{d}{55 \rho} }$.
 
 According to the definition of $\bar{\gamma} = \min_k \gamma_k$, we have
  \begin{align}\label{eq: min_gam_ave}
     \bar \gamma \geq & \frac{\eta}{2} - \frac{c_0}{2 \beta} \eta - \eta^2 L \frac{(36+2b)(q+d)}{bq}  - \eta^2 c_0 \frac{(72+4b)(q+d)}{bq}.
 \end{align}
 
 
  From \eqref{eq: ck_upper_ave} and the definition of $\beta$, we have
 \begin{align}\label{eq: c0_beta_ave}
     \frac{c_0}{2\beta} \leq \frac{27\rho}{b \min\{d,q\}}. %\leq 15 c.
 \end{align}
 Since $\eta = \rho/(Ld)$, we have
 \begin{align}\label{eq: eta_L_ave}
     \eta L  \frac{(36+2b)(q+d)}{bq}  \leq \frac{2\rho}{\min\{ d,q\}} \left (\frac{36}{b} +2 \right ),
 \end{align}
 where we used the fact that $\frac{1}{d} + \frac{1}{q } \leq \frac{2}{\min\{ d,q\}}$. Moreover, we have
  \begin{align}\label{eq: eta_c0_ave}
     \eta c_0   \frac{(72+4b)(q+d)}{bq} \leq  &
     \frac{\rho}{L}\frac{54L  \rho}{b \min\{ q,d\}}  \left (4 + \frac{72}{b} \right ) \left (\frac{1}{d}+ \frac{1}{q} \right ) \nonumber \\
    \leq  & \frac{108 \rho^2}{b \min\{ d,q\}^2} \left (4 + \frac{72}{b} \right )
 \end{align}
Substituting \eqref{eq: c0_beta_ave}-\eqref{eq: eta_c0_ave} into \eqref{eq: min_gam_ave}, and following the arguments in \eqref{eq: gamma_bar_bound}, we   obtain 
\begin{align}\label{eq: gamma_bar_bound_ave}
     \bar \gamma \geq & 
      \alpha_0 \eta,
 \end{align}
where $\alpha_0 > 0$  is a universal constant that is   independent of $T$, $d$ and $b$.
 

Based the definition of $\chi_k$, the upper bound on $\chi_m = \sum_k \chi_k$ is given by
 \begin{align}
     \chi_m \leq  &  \eta m  \left (1-  \frac{c_{0} }{\beta} \right ) \frac{\mu^2 d^2 L^2}{4} +
    \eta m \left ( \frac{L}{2}  + c_{0} \right )\frac{ (6+b)(q+1) L^2 d^2 \mu^2 + 72 (q+d) \sigma^2 }{bq} \eta .
 \end{align}
Using \eqref{eq: ck_upper_ave} and assuming $b \geq 18$ (without loss of generality), then
 $
 \frac{L}{2} + c_0 \leq \frac{L}{2} + 54 L \rho b^{-1}  \leq \frac{7 L}{2}
 $. This yields
 \begin{align}
     \frac{\chi_m}{\bar \gamma} \leq&
 \frac{m}{\alpha_0} \frac{d^2 L^2 }{4} \frac{1}{dT}  + \frac{m}{\alpha_0} 
   \frac{7L}{2} \frac{(6+b)(q+1)L^2 d^2}{bq} \frac{1}{dT} \frac{\rho}{Ld } +  \frac{m}{\alpha_0} \frac{7L}{2} \frac{72 \sigma^2}{b} \left(\frac{1}{d} + \frac{1}{q} \right ) \rho \nonumber \\
   \leq & O \left (
   \frac{md}{T}  + \frac{m}{b \min\{d,q \}}
   \right )
 \end{align}
Since  $T = S m$, we have
 \begin{align}\label{eq: const_error_bd_ave}
     \frac{S\chi_m}{ T \bar \gamma} \leq O \left (
\frac{d}{T} + \frac{1}{b \min\{d,q\}}
\right ).
 \end{align}

 
 Substituting \eqref{eq: gamma_bar_bound_ave} and 
 \eqref{eq: const_error_bd_ave} into \eqref{eq: grad_norm_SVRG}, we have
\begin{align} \label{eq: grad_norm_SVRG_ave_special}
    \mathbb E[ \| \nabla f(\bar { \mathbf x }) \|_2^2 ] \leq &
\frac{[f(\tilde{\mathbf x}_0) - f^*]}{T \alpha_0 }
\frac{L d}{ \rho }
+   \frac{L^2 }{T^2 \alpha_0 \rho}
+ \frac{S\chi_m }{ T \bar \gamma} = O\left ( 
\frac{ d}{T} + \frac{1}{b \min\{d,q \}}
\right ).
\end{align}


 \hfill $\square$
 
 
 \subsection{Proof of Theorem~\ref{thr: ZO_SVRG_coord}} \label{supp: thr3}

 
 Since $f$ is $L$-smooth, we have
\begin{align}\label{eq: fsmooth_def_SVRG_coord}
f (\mathbf x_{k+1}^s) \leq & f (\mathbf x_k^s) - \eta_k \inp{\nabla f (\mathbf x_k^s)  }{\hat {\mathbf v}_k^s}  + \frac{L}{2} \eta_k^2 \| \hat {\mathbf v}_k^s \|_2^2.
\end{align}
Since $\mathbf x_{k}^s$ and $\mathbf x_0^s$  are independent of $\mathcal I_{k}$  used in $\hat \nabla f_{\mathcal I_{k}} (\mathbf x_{k}^s)$ and $\hat \nabla f_{\mathcal I_{k}} (\mathbf x_{0}^s)$,  we obtain
\begin{align}\label{eq: E_uIk_v_coord}
    \mathbb E_{ \mathcal I_{k}} [\mathbf v_{k}^s]  &  =   \hat \nabla f(\mathbf x_{k}^s)  + \hat \nabla  f (\mathbf x_0^s) - \hat \nabla f (\mathbf x_0^s)   =  \hat \nabla f(\mathbf x_{k}^s),
\end{align}
where we recall that a deterministic gradient estimator is used.
Combining \eqref{eq: fsmooth_def_SVRG_coord} and \eqref{eq: E_uIk_v_coord}, we have
\begin{align}\label{eq: fsmooth_def_SVRG2_coord}
 \mathbb E \left [ f (\mathbf x_{k+1}^s)  \right ] 
 \leq & \mathbb E \left [ f (\mathbf x_k^s)  \right ] - \eta_k \mathbb E \left [ \inp{\nabla f(\mathbf x_k^s)}{\hat \nabla f(\mathbf x_k^s)} \right ] + \frac{L}{2} \eta_k^2 \mathbb E \left [  \| \hat {\mathbf v}_k^s \|_2^2 \right ].   
\end{align}

 In \eqref{eq: fsmooth_def_SVRG2_coord}, we   bound $ -2 \mathbb E \left [ \inp{\nabla f(\mathbf x_k^s)}{\hat \nabla f(\mathbf x_k^s)} \right ]$ as,
\begin{align}\label{eq: prod_est_coord} 
 -2  \mathbb E \left [ \inp{\nabla f (\mathbf x_k^s)}{\hat{\nabla} f (\mathbf x_k^s)} \right ] 
\leq  & \mathbb E \left [ \|  {\nabla} f  ( {\mathbf x}_{k}^s) - \hat {\nabla} f  ( {\mathbf x}_{k}^s)  \|_2^2 \right ] - \left [ \mathbb E \| \nabla f(\mathbf x_k^s) \|_2^2 \right ] \nonumber \\
\overset{\eqref{eq: grad_diff_allcoord}}{\leq}
  & \frac{L^2 d^2 \mu^2}{4}
  - \mathbb E \left [ \| \nabla f(\mathbf x_k) \|_2^2 \right ],
%\leq & \frac{L^2 d}{2 b} \sum_{\ell = 1}^d \mu_\ell^2 - \| \nabla f(\mathbf x_k) \|_2^2,
\end{align}
where the first inequality holds since $-2 \inp{\mathbf a}{\mathbf b} \leq \| \mathbf a - \mathbf b \|_2^2 - \| \mathbf a \|_2^2$.

Substituting \eqref{eq: prod_est_coord} into \eqref{eq: fsmooth_def_SVRG2_coord}, we have
\begin{align}\label{eq: fsmooth_def_SVRG2_coord2}
  \mathbb E \left [ f (\mathbf x_{k+1}^s) \right ]  
 \leq & \mathbb E \left [ f (\mathbf x_k^s) \right ] - \frac{\eta_k}{2} \mathbb E \left [ \| \nabla f(\mathbf x_k) \|_2^2 \right ]  + \frac{L}{2} \eta_k^2 \mathbb E\left [ \| \hat{\mathbf v}_k^s \|_2^2 \right ]   + \frac{L^2 d^2 \mu^2 \eta_k}{8}.   
\end{align}



In \eqref{eq: fsmooth_def_SVRG2_coord2}, we next bound $\mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ] $.
Following \eqref{eq: E_Iv_v}-\eqref{eq: vks_norm_SVRG}, we have
 \begin{align}\label{eq: vks_norm_SVRG_coord0}
      \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ]  \leq 
      & \frac{2}{b} \mathbb E \left [ \| \hat \nabla f_{i}(\mathbf x_k^s) - \hat \nabla f_{i}(\mathbf x_0^s)  \|_2^2 \right ]   + 2 \mathbb E \left [\|\hat \nabla f(\mathbf x_k^s) \|_2^2  \right ].
 \end{align}
 The first term at RHS of \eqref{eq: vks_norm_SVRG_coord0} yields
  \begin{align} \label{eq: dist_est_twopoint_coord}
  &  \mathbb E \left [ \| \hat \nabla f_{i} ( \mathbf x_k^s ) - \hat \nabla f_{i} ( \mathbf x_0^s ) \|_2^2 \right   ]  \overset{\eqref{eq: grad_f_smooth_coord_all}}{=} \mathbb E \left [ \left \|  \sum_{\ell=1}^d \left  ( \frac{\partial f_{i,\mu_\ell}}{ \partial x_{k,\ell}^s }\mathbf e_\ell -\frac{\partial f_{i,\mu_\ell}}{ \partial x_{0,\ell}^s } \mathbf e_\ell  \right )  \right \|_2^2 \right ] \nonumber \\
\overset{\eqref{eq: sum_exp_bd}}{\leq}  & d  \sum_{\ell=1}^d \mathbb E \left [\left  \|   \frac{\partial f_{i,\mu_\ell}}{ \partial x_{k,\ell}^s }  - \frac{\partial f_{i,\mu_\ell}}{ \partial x_{0,\ell}^s } \right \|_2^2 \right ]
  \leq  L^2 d \sum_{\ell = 1}^d \mathbb E \left [ \| x_{\ell,k}^s - x_{\ell,0}^s \|_2^2 \right ] = L^2 d \mathbb E \left [ \| \mathbf x_{k}^s - \mathbf x_{0}^s \|_2^2 \right ],
 \end{align}
 where   $ f_{i,\mu_\ell} (\mathbf x) = \mathbb E_{u \sim U [-\mu_\ell, \mu_\ell]} f_i(\mathbf x + u \mathbf e_\ell)$ denotes the smooth function of $f_i$ with respect to its $\ell$th coordinate   (Lemma\,\ref{lemma: deter_smooth_gradest}), $x_{k,\ell}^s$ denotes the $\ell$th coordinate of $\mathbf x_k^s$,
 $\frac{\partial f_{i,\mu_\ell}}{ \partial x_{k,\ell}^s }$ is the $\ell$th partial derivative of $f_{i,\mu_\ell}$  at   $\mathbf x_k^s$, and
 the second inequality holds since $f_{i,\mu_\ell}(\mathbf x)$ is $L$-smooth (Lemma\,\ref{lemma: deter_smooth_gradest}) with respect to the $\ell$th coordinate.
From \eqref{eq: grad_diff_allcoord}, the second term at RHS of  \eqref{eq: vks_norm_SVRG_coord0} yields
\begin{align}\label{eq: grad_est_norm_deter_sig}
    \| \hat \nabla f(\mathbf x) \|_2^2 & \leq 2 \| \nabla f(\mathbf x) \|_2^2 + 2 \|  \hat{\nabla} f(\mathbf x) - \nabla f(\mathbf x)   \|_2^2    \overset{\eqref{eq: grad_diff_allcoord}}{\leq} 2 \| \nabla f(\mathbf x) \|_2^2 + \frac{L^2 d^2 \mu^2}{2},
\end{align}
where we used the fact that $\mu_\ell = \mu$.
 
 Substituting
 \eqref{eq: dist_est_twopoint_coord}
 and
 \eqref{eq: grad_est_norm_deter_sig}
 into  \eqref{eq: vks_norm_SVRG_coord0}, we have 
 \begin{align}\label{eq: vks_norm_SVRG_coord}
     & \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ] \leq 
    \frac{2 L^2 d}{b} \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ]
    +  4 \mathbb E \left [ \| \nabla f(\mathbf x) \|_2^2 \right ] + L^2 d^2 \mu^2.
   % \leq & \frac{2}{b} \mathbb E [ \| \hat \nabla f_{i_k} ( \mathbf x_k^s ) - \hat \nabla f_{i_k} ( \mathbf x_0^s )   \|_2^2] + 2 \mathbb E [\|\hat \nabla f(\mathbf x_k^s) \|_2^2  ],
 \end{align}
 
 Similar to \eqref{eq: norm_xk_dif}, we have
 \begin{align}\label{eq: norm_xk_dif_coord}
& \mathbb E \left [\| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2 \right ] 
  \leq  \eta_k^2 \mathbb E \left [
   \| \hat {\mathbf v}_{k}^s\|_2^2
   \right ] + \mathbb E \left [
   \|
  \mathbf x_{k}^s - \mathbf x_0^s
  \|_2^2
   \right ]
   + \eta_k\mathbb E \left [
  \frac{1}{\beta_k}   \| \hat \nabla f(\mathbf x_{k}^s) \|_2^2 +  \beta_k  \| \mathbf x_{k}^s - \mathbf x_0^s \|_2^2
  \right ] \nonumber \\
&  \overset{\eqref{eq: grad_est_norm_deter_sig}}{\leq} 
\eta_k^2 \mathbb E \left [
   \| \hat {\mathbf v}_{k}^s\|_2^2
   \right ] + \mathbb E \left [
   \|
  \mathbf x_{k}^s - \mathbf x_0^s
  \|_2^2
   \right ]
   + \eta_k\mathbb E \left [
  \frac{2}{\beta_k}   \| \nabla f(\mathbf x_{k}^s) \|_2^2 +  \beta_k  \| \mathbf x_{k}^s - \mathbf x_0^s \|_2^2
  \right ]   + \frac{L^2 \mu^2 d^2 \eta_k}{\beta_k 2}.
\end{align}
Define the following   Lyapunov function,
\begin{align}\label{eq: Def_Rks_coord}
    R_{k}^s = \mathbb E \left [ f  (\mathbf x_k^s) + c_k \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ],
\end{align}
where $c_k > 0 $.

Based on \eqref{eq: fsmooth_def_SVRG2_coord2}  and \eqref{eq: norm_xk_dif_coord}, we obtain
\begin{align}
\label{eq: Rk_new_SCRG_coord}
    R_{k+1}^s  
    =  & \mathbb E \left [ f (\mathbf x_{k+1}^s) + c_{k+1} \| \mathbf x_{k+1}^s - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   \leq
    & \mathbb E [ f (\mathbf x_k^s)] - \left ( \frac{\eta_k}{2}-  \frac{c_{k+1} \eta_k}{2\beta_k} \right ) \mathbb E \left [ \| \nabla f (\mathbf x_k^s) \|_2^2 \right ]   + (c_{k+1} + c_{k+1} \beta_k \eta_k) \mathbb E \left [ \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \mathbb E \left [ \| \hat {\mathbf v}_k^s \|_2^2 \right ]   + \frac{d^2 L^2 \mu^2 \eta_k}{8}+ \frac{d^2 L^2 \mu^2  c_{k+1} \eta_k}{2 \beta_k}.
\end{align}
Substituting 
\eqref{eq: vks_norm_SVRG_coord} into \eqref{eq: Rk_new_SCRG_coord}, we have
\begin{align}
\label{eq: Rk_new_SCRG_2_coord}
   R_{k+1}^s  
  \leq &   \mathbb E \left [ f (\mathbf x_k^s) \right ] - \left ( \frac{\eta_k}{2}-  \frac{c_{k+1} \eta_k}{2\beta_k} \right ) \mathbb E \left [ \| \nabla f (\mathbf x_k^s) \|_2^2 \right ]   + (c_{k+1} + c_{k+1} \beta_k \eta_k) \mathbb E \left [ \| \mathbf x_k^{s} - \mathbf x_0^s \|_2^2 \right ] \nonumber \\
   & + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right )\frac{2L^2d}{b} \mathbb E \left [ \| \mathbf x_k^s - \mathbf x_0^s \|_2^2 \right ]   + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) 4 \mathbb E \left [ \| \nabla f  (\mathbf x_k^{s}) \|_2^2 \right ] \nonumber \\ 
& + \left ( \frac{L}{2} \eta_k^2 + c_{k+1} \eta_k^2 \right ) \mu^2 L^2 d^2   + \frac{d^2 L^2 \mu^2 \eta_k}{8}+ \frac{d^2 L^2 \mu^2  c_{k+1} \eta_k}{2 \beta_k}.
\end{align}

Based on the definition of $c_k$, i.e.,
\begin{align*}
    c_k =& \left ( 1 +   \beta_k \eta_k + \frac{2d L^2 \eta_k^2}{b}  \right )  c_{k+1} + \frac{ d L^3 \eta_k^2}{b},
\end{align*}
we can simplify \eqref{eq: Rk_new_SCRG_2_coord} to
\begin{align}
\label{eq: Rk_new_SCRG_2_2_coord}
   R_{k+1}^s  
\overset{ \eqref{eq: Def_Rks_coord}}{\leq} 
  R_k^s - \gamma_k \mathbb E [ \| \nabla f (\mathbf x_k^s) \|_2^2 ]  + \chi_k,
\end{align}
where we recall that
\begin{align*}
\gamma_k = & 
\frac{1}{2}\left( 1 - \frac{c_{k+1}}{\beta_k} \right ) \eta_k - 4\left(
\frac{L}{2} + c_{k+1}
\right ) \eta_k^2, \nonumber \\
\chi_k =  & 
\frac{1}{2}\left( \frac{1}{4} + \frac{c_{k+1}}{\beta_{k+1}} \right) L^2 d^2 \mu^2 \eta_k
+ \left (\frac{L}{2} + c_{k+1} \right ) \mu^2 L^2 d^2  \eta_k^2.
\end{align*}

Based on \eqref{eq: Rk_new_SCRG_2_2_coord}
and following the similar argument in \eqref{eq: Rk_new_SCRG_4}-\eqref{eq: grad_mid_Sm}, we have 
 \begin{align*}
     \sum_{s=1}^S \sum_{k=0}^{m-1}\gamma_k  \mathbb E[\| \nabla f(\mathbf x_k^s) \|_2^2] 
   \leq \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ]  + S \chi_m.
\end{align*}
Consider $\bar{\gamma} = \min_k \gamma_k$ and the distribution of choosing $\bar{\mathbf x}$, we obtain
\begin{align}
       \mathbb E[\| \nabla f(\bar {\mathbf x}) \|_2^2]  
    \leq     \frac{ \mathbb E[  f(\tilde {\mathbf x}_{0}) - f^* ] }{T \bar \gamma} + \frac{S \chi_m}{T \bar \gamma}.
\end{align}


The rest of the proofs essentially follow along the lines of Corollary\,\ref{col: SVRG_simple} under a different parameter setting.

Since $c_k = c_{k+1} (1+ \theta)  + \frac{dL^3 \eta^2}{b} $, we 
have   $ c_k \leq c_0$ for any $k$, and  $\theta =  \beta \eta + \frac{2dL^2  \eta^2}{b}$. This yields
\begin{align}\label{eq: c0_coord}
    c_0 & = \frac{dL^3 \eta^2}{b} \frac{(1+ \theta)^m - 1}{\theta}.
\end{align}
When $\eta = \rho/(Ld)$ and $\beta = L$ we have 
\begin{align}\label{eq: theta_coord}
    \theta = \frac{\rho}{ d} +   \frac{2  \rho^2 }{  b d} \leq \frac{3 \rho }{ d}.
\end{align}
Substituting \eqref{eq: theta_coord} into \eqref{eq: c0_coord}, we have
\begin{align}\label{eq: ck_upper_coord}
   c_k \leq c_0 & = \frac{d L^3}{b} \frac{\eta^2}{\theta } [(1+ \theta)^m - 1]   = \frac{\rho L}{b + 2 \rho}  [(1+ \theta)^m - 1]   \leq \frac{L \rho}{b} (e - 1) \leq \frac{2L \rho}{b},
 \end{align}
 where the second equality holds similar to  \eqref{eq: ck_upper} under $m = \ceil{\frac{d}{3 \rho} }$.
 
 Based on \eqref{eq: ck_upper_coord} and the definition of $\bar{\gamma}$, similar to \eqref{eq: c0_beta}-\eqref{eq: gamma_bar_bound} we can obtain
 \begin{align}\label{eq: gamma_bar_bound_coord}
     \bar \gamma \geq & 
      \eta \alpha_0,
 \end{align}
where $\alpha_0 > 0$   is independent of $T$, $d$ and $b$.


Since $\chi_m = \sum_k \chi_k $, it can be bounded as 
 \begin{align}
     \chi_m \leq  & m \eta^2   \left (\frac{L}{2} + c_0 \right ) \mu^2 L^2 d^2 + m \eta \frac{d^2 L^2 \mu^2 }{8}  + m \eta \frac{d^2 L^2 \mu^2  c_{0} }{2 \beta}.
 \end{align}
 From \eqref{eq: ck_upper_coord}, we have   
 $
 \frac{L}{2} + c_0 \leq \frac{L}{2} + 2 L \rho b^{-1}  \leq \frac{5 L}{2}
 $.  
Moreover, based on  $T = S m$ and  $\mu = \frac{1}{\sqrt{d}\sqrt{T}}$, we have
 \begin{align}\label{eq: const_error_bd_coord}
     \frac{S\chi_m}{ T \bar \gamma} \leq&
    \frac{5 L^2 \rho }{2 \alpha_0 T }  +
     \frac{dL^2}{8 \alpha_0 T}   +  \frac{d \rho L^2}{\alpha_0 bT} = O \left ( \frac{1}{T} + 
\frac{d }{T}   + \frac{d }{bT}
\right ),
 \end{align}
 where in the big $O$ notation, we  ignore the constant numbers that are independent of $L$, $d$, $b$, and $T$.
 
 Substituting \eqref{eq: gamma_bar_bound_coord} and 
 \eqref{eq: const_error_bd_coord} into \eqref{eq: grad_norm_SVRG_coord}, we have
\begin{align} \label{eq: grad_norm_SVRG_special_coord}
    \mathbb E[ \| \nabla f(\bar { \mathbf x }) \|_2^2 ] \leq &
\frac{[f(\tilde{\mathbf x}_0) - f^*]}{T \alpha_0 }
\frac{L d}{ \rho }
+ \frac{S \chi_m }{ T \bar \gamma}  
= O\left ( 
\frac{d}{T}  
\right ).
\end{align}

 \hfill $\square$
 
 \subsection{Auxiliary Lemmas}\label{app: aux}
 
 \begin{mylemma}\label{lemma: minibatch}
Let $\{ \mathbf z_i \}_{i=1}^n$ be an arbitrary sequence of $n$ vectors. Let $\mathcal I$ be a mini-batch of size $b$, which contains i.i.d. samples selected uniformly randomly (with replacement) from  $[n]$. Then
\begin{align}\label{eq: exp_minibatch_2}
    \mathbb E_{\mathcal I}\left [  \frac{1}{b} \sum_{i \in \mathcal I} \mathbf z_i    \right ]  
 = \mathbb E[\mathbf z_i]  =  \frac{1}{n}\sum_{j=1}^n \mathbf z_j.
\end{align}
When $\mathbb E [\mathbf z_i] = \mathbf 0$, then
\begin{align}\label{eq: exp_minibatch_special}
     \mathbb E_{\mathcal I}\left [ \left \|  \frac{1}{b} \sum_{i \in \mathcal I} \mathbf z_i \right \|_2^2 \right ]  = \frac{1}{b} \mathbb E [\| \mathbf z_i \|_2^2]
 = \frac{1}{bn}\sum_{i=1}^n \| \mathbf z_i \|_2^2.
\end{align}
\end{mylemma}

\textbf{Proof:}
Based on the definition of $\mathcal I$, we immediately obtain
$
    \mathbb E_{\mathcal I}\left [  \frac{1}{b} \sum_{i \in \mathcal I} \mathbf z_i    \right ]  
 = \mathbb E[ \mathbf z_i] = \frac{1}{n}\sum_{j=1}^n \mathbf z_j$.

Since $\mathbb E[\mathbf z_i \mathbf z_j] = \mathbb E[\mathbf z_i] \mathbb E[\mathbf z_j] = \mathbf 0$ for $i \neq j$,  we have
\begin{align}\label{eq: exp_z}
    \mathbb E \left [ \left \|  \frac{1}{b} \sum_{i \in \mathcal I} \mathbf z_i \right \|_2^2 \right ]
 =  &  \frac{1}{b^2} 
 \sum_{i \in \mathcal I} \mathbb E[ \| \mathbf z_i \|_2^2] = \frac{1}{b} \mathbb E[ \| \mathbf z_i \|_2^2] = \frac{1}{bn}\sum_{i=1}^n \| \mathbf z_i \|_2^2.  
\end{align}
The proof is now complete.
\hfill $\square$

\begin{mylemma}\label{lemma: sum_exp_bd}
For  variables $\{ \mathbf z_i \}_{i=1}^n$, we have
%{\color{green} Do we really need this lemma as it trivially follows from Jensen's inequality}
\begin{align}\label{eq: sum_exp_bd}
 \left \| \sum_{i=1}^n \mathbf z_i \right  \|_2^2  \leq n \sum_{i=1}^n  \| \mathbf z_i \|_2^2.
\end{align}
\end{mylemma}
\textbf{Proof}: Since $\phi(\mathbf x) = \| \mathbf x \|_2^2$ is convex, the 
 Jensen's inequality yields $\| \frac{1}{n} \sum_i \mathbf z_i \|_2^2 \leq \frac{1}{n} \sum_i \| \mathbf z_i \|_2^2$.
 \hfill $\square$

\begin{mylemma}\label{lemma: Lsmooth_v2}
if $f$ is $L$-smooth, then for any $\mathbf x, \mathbf y \in \mathbb R^d$
\begin{align}\label{eq: Lsmooth_v2}
    | f(\mathbf x) - f(\mathbf y) - \inp{\nabla f_i(\mathbf y)}{\mathbf x - \mathbf y} | \leq \frac{L}{2} \| \mathbf x - \mathbf y \|_2^2.
\end{align}
\end{mylemma}
 \textbf{Proof}: This is a direct consequence of A2 \citep{lei2017non}. \hfill $\square$
 
\subsection{Application: black-box classification}
\label{supp: experiment_classification}
\paragraph{Real dataset}
Our dataset consists of 
 $N = 1000$ crystalline materials/compounds, each of which corresponds to a numerical valued feature vector $\mathbf a_i$. The feature vector encodes chemical information regarding constituent elements. There exist $d=145$ attributes, such as, stoichiometric properties, elemental statistics, electronic structure properties attributes, and ionic compound attributes \citep{magpie}. The label information  $y_i\in \{0,1\}$ (conductor against insulator)  is determined using DFT calculations \citep{vasp}. We equally divided the data into a training and test set.
 
\paragraph{Parameter setting}
In our ZO algorithms, unless specified otherwise, 
the length of each epoch is set by $m = 50$, the mini-batch size is $b = 10$, the number of random direction samples is $q = 10$, the initial value is given by 
 $\tilde{\mathbf x}_0 = \mathbf 0$, and the smoothing parameter  follows
$
\mu = O( 1/\sqrt{dT} )
$. 
%For SGD, we   choose $\eta = 0.1$.  
% For SVRG, we choose
% $\eta = O( {b}/{n^{\frac{2}{3}}} )$ suggested by   \cite[Theorem\,7]{reddi2016stochastic}. 
For ZO-SGD, ZO-SVRC and ZO-SVRG, we choose
$
\eta = O( 1/d )
$ suggested by  Corollary \ref{col: SVRG_simple} and \citep[Corollary\,3.3]{ghadimi2013stochastic}. 
Also ZO-SVRC updates $J=1$ coordinates per iteration within an epoch.
%where $\alpha = 0.8$. 


\subsection{Application: generating universal adversarial perturbations from black-box DNNs} 
\label{appendix: adv_app}
\paragraph{Problem formulation}
In image classification, adversarial examples refer to carefully crafted perturbations such that, when added to the natural images, are visually imperceptible but will lead the target model to misclassify.
When testing the robustness of a deployed black-box DNN (e.g., an online image classification service), the model parameters are hidden and acquiring its gradient is inadmissible. But one has access to the input-output correspondence of the target model  $F(\cdot)$, rendering generating adversarial examples a ZO optimization problem. 

We consider the task of generating a universal perturbation to a batch of $n = 10$ images via iteratively querying the target DNN. These images are selected from the class of digit ``1'' and are all originally correctly classified by the DNN. In problem \eqref{eq: prob_ori}, let $f_i(\mathbf x)= c \cdot \max \{ F_{y_i} (0.5 \cdot \tanh ( \tanh^{-1} 2 \mathbf  a_i + \mathbf x)) - \max_{j \neq y_i} F_j(0.5 \cdot \tanh ( \tanh^{-1} 2 \mathbf a_i + \mathbf x)) , 0 \} + \|0.5 \cdot \tanh ( \tanh^{-1} 2 \mathbf a_i + \mathbf x) - \mathbf a_i \|_2^2  $ be the designed attack loss function of the $i$th image \cite{chen2017zoo,carlini2017towards}. 
Here  $(\mathbf a_i,y_i)$ denotes the pair of the $i$th natural image $\mathbf a_i \in [-0.5,0.5]^d$ and its original class label $y_i$. The function $F(\mathbf z)=[F_1(\mathbf z),\ldots,F_K(\mathbf z)]$ outputs the model prediction scores (e.g., log-probabilities) of the input $\mathbf z$ in  all $K$ image classes.
The $\tanh$ operation ensures the generated adversarial example $0.5 \cdot \tanh ( \tanh^{-1} \mathbf a_i + \mathbf x)$ still lies in the valid image space $[-0.5,0.5]^d$.  The regularization parameter $c$  trades off adversarial success and the $\ell_2$ distortion of adversarial examples. In our experiment, we set $c = 1$ and use the log-probability as the model output. 
The reported $\ell_2$ distortion is the least averaged distortion over the $n$ successful adversarial images relative to the original images among the $S$ iterations.

\paragraph{Generated adversarial images}
Table \ref{table:digit1} displays the original images and their adversarial examples generated by ZO-SGD and ZO-SVRG. Their statistics  are given in Fig. \ref{Fig3}. Table \ref{table:digit4} shows another visual comparison chart of digit class ``4''.

% The regularization parameter $c$  trades off adversarial success and $\ell_2$ distortion, $F(\mathbf z)=[F_1(\mathbf z),\ldots,F_K(\mathbf z)]$ outputs the model prediction scores (e.g., log-probabilities) of the input $\mathbf z$ in  all $K$ image classes, and $(\mathbf a_i,y_i)$ denotes the pair of the $i$th natural image $\mathbf a_i \in [-0.5,0.5]^d$ and its original class label $y_i$. The $\tanh$ operation ensures the generated adversarial example $0.5 \cdot \tanh ( \tanh^{-1} \mathbf a_i + \mathbf x)$ still lies in the valid image space $[-0.5,0.5]^d$.

\begin{table*}
  [ht] \caption{Comparison of generated adversarial examples from a black-box DNN on MNIST: digit class ``1''.} \label{table:digit1}
  \begin{adjustbox}{max width=\textwidth }
  \begin{tabular}
      {ccccccccccc}
      \hline
      	Image ID & 2 & 5 & 14 & 29 & 31 & 37 & 39 & 40 & 46 & 57 \\
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	Original &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0002.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0005.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0014.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0029.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0031.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0037.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0039.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0040.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0046.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0057.png}}
      \vspace{0.2cm} \\
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SGD} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id2_Orig1_Adv7_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id5_Orig1_Adv7_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id14_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id29_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id31_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id37_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id39_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id40_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id46_Orig1_Adv3_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id57_Orig1_Adv7_ZOSGD.png}} \\
        Classified as & 7 & 7 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 7 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 10} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id2_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id5_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id14_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id29_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id31_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id37_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id39_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id40_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id46_Orig1_Adv3_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id57_Orig1_Adv3_ZOSVRG.png}} \\
        Classified as & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 20} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id2_Orig1_Adv7_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id5_Orig1_Adv7_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id14_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id29_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id31_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id37_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id39_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id40_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id46_Orig1_Adv3_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id57_Orig1_Adv7_ZOSVRGq20.png}} \\
        Classified as & 7 & 7 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 7 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 30} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id2_Orig1_Adv7_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id5_Orig1_Adv7_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id14_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id29_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id31_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id37_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id39_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id40_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id46_Orig1_Adv3_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id57_Orig1_Adv7_ZOSVRGq30.png}} \\
        Classified as & 7 & 7 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 7 \\
      \hline
  \end{tabular}
  \end{adjustbox}
\end{table*}
 

\begin{table*}
  [ht] \caption{Comparison of generated adversarial examples from a black-box DNN on MNIST: digit class ``4''.} \label{table:digit4}
  \begin{adjustbox}{max width=\textwidth}
  \begin{tabular}
      {ccccccccccc}
      \hline
      	Image ID & 4 & 6 & 19 & 24 & 27 & 33 & 42 & 48 & 49 & 56 \\
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	Original &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0004.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0006.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0019.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0024.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0027.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0033.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0042.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0048.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0049.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{0056.png}}
      \vspace{0.2cm} \\
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SGD} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id4_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id6_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id19_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id24_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id27_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id33_Orig4_Adv2_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id42_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id48_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id49_Orig4_Adv9_ZOSGD.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id56_Orig4_Adv9_ZOSGD.png}} \\
        Classified as & 9 & 9 & 9 & 9 & 9 & 2 & 9 & 9 & 9 & 9 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 10} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id4_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id6_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id19_Orig4_Adv7_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id24_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id27_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id33_Orig4_Adv5_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id42_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id48_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id49_Orig4_Adv9_ZOSVRG.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id56_Orig4_Adv9_ZOSVRG.png}} \\
        Classified as & 9 & 9 & 7 & 9 & 9 & 5 & 9 & 9 & 9 & 9 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 20} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id4_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id6_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id19_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id24_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id27_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id33_Orig4_Adv5_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id42_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id48_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id49_Orig4_Adv9_ZOSVRGq20.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id56_Orig4_Adv9_ZOSVRGq20.png}} \\
        Classified as & 9 & 9 & 9 & 9 & 9 & 5 & 9 & 9 & 9 & 9 \\
      \hline
      
      \hline &&&&&&&&&& \vspace{-0.2cm} \\
      	\thead{ZO-SVRG\\q = 30} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id4_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id6_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id19_Orig4_Adv7_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id24_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id27_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id33_Orig4_Adv0_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id42_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id48_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id49_Orig4_Adv9_ZOSVRGq30.png}} &
        \parbox[c]{2.2em}{\includegraphics[width=0.4in]{Adv_id56_Orig4_Adv9_ZOSVRGq30.png}} \\
        Classified as & 9 & 9 & 7 & 9 & 9 & 0 & 9 & 9 & 9 & 9 \\
      \hline
  \end{tabular}
  \end{adjustbox}
\end{table*}
